Scoring Play Combinatorial Games Under Different Operators

Scoring play games were first studied by Fraser Stewart for his PhD thesis. He showed that under the disjunctive sum, scoring play games are partially ordered, but do not have the same "nice" structure of normal play games. In this paper I will be considering scoring play games under three different operators given by John Conway and William Stromquist and David Ullman, namely the conjunctive sum, selective sum and sequential join.

==> cg-base.tex <==
\ProvidesFile{cg-base.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                          %%
%%              Raymond Chen's Game Builder                 %%
%%                  (somewhat altered)                      %%
%%                                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The \combgame macro takes as its argument the description of a game.
% It measures the size of the contents and scales all the slashes
% inside to the proper size.
%
% This makes eight passes over the input argument.
%
% For each of the four typestyles...
%
%   Typeset the argument in that style.
%   Set \cg@gamebox to an empty box with the height and depth of the game.
%       (During this first pass, \ifcg@drawbars is \iffalse.)
%   If we are in display style, set \cg@extension to the size of the
%       delimiter extension.  (If not, then set it to zero.)
%   Typeset the game proper, setting \ifcg@drawbars to \iftrue.
%
% This macro requires cooperation from the \cgslash, \cgsslash, etc. macros.

\newmuskip\cgslashmuskip
\cgslashmuskip=-2mu
\newlength\cgslashextension
\setlength\cgslashextension{1.5pt}

\def\cg@slashskip{\mskip\cgslashmuskip}

\newif\ifcg@star
\newif\ifcg@building\cg@buildingfalse
\newif\ifcg@drawbars\cg@drawbarsfalse
\newbox\cg@gamebox\setbox\cg@gamebox=\null
\newdimen\cg@extension
\newcounter{cg@readbarctr}

\newcommand\combgame{%
  \begingroup%
  \catcode`\|=\active%
  \cg@definebars%
  \@ifstar{\cg@startrue\cg@combgame}{\cg@starfalse\cg@combgame}%
}

\def\cg@combgame#1{%
  \mathpalette\cg@buildgame{#1}%
  \endgroup%
}

\def\cg@buildgame#1#2{%
    \begingroup%
    \cg@buildingtrue%
    \ifx#1\displaystyle%
      \ifcg@star%
        \cg@extension=0pt%
      \else%
        \cg@extension=\the\cgslashextension%
      \fi%
    \fi%
    \cg@drawbarsfalse%
    \setbox\z@\hbox{$#1#2$}%
    \ht\cg@gamebox\ht\z@%
    \dp\cg@gamebox\dp\z@%
    \cg@drawbarstrue%
    #1{#2}%
    \cg@buildingfalse%
    \endgroup%
}

\begingroup
\catcode`\|=\active
\gdef\cg@definebars{%
  \def|{\setcounter{cg@readbarctr}{1}\cg@readbars}%
  \def\{{\left\lbrace}
  \def\}{\right\rbrace}
}
\gdef\cg@readbars{%
  \@ifnextchar|{\stepcounter{cg@readbarctr}\cg@readnextbar}{\cgslashes{\thecg@readbarctr}}%
}
\gdef\cg@readnextbar|{\cg@readbars}
\endgroup

\newcommand\cgslash{\cgslashes{1}}
\newcommand\cgsslash{\cgslashes{2}}

\newcommand\cgslashes[2][]{%
  \ifcg@building
    \ifcg@drawbars
        \mathrel
        {\hbox{$%
    %% This part is deadly because \left and \right create implicit
    %% grouping.
        \toks\z@{}%
        \cg@loopmbars{#2}{\global\toks\z@\expandafter{\the\toks\z@\cg@mbarshelper}}%
        \def\cg@mbarshelper{\left\vert\mskip\cgslashmuskip}\the\toks\z@
            \mskip-\cgslashmuskip
            \@tempcnta#2\relax \advance\@tempcnta\m@ne
            \raise\@tempcnta\cg@extension\copy\cg@gamebox
            \lower\@tempcnta\cg@extension\copy\cg@gamebox
        \gdef\cg@mbarshelper{\right.}\the\toks\z@\n@space$}}%
    \else\mathrel\vert\fi
  \else
    \cg@badbar
  \fi
}

\def\cg@loopmbars#1#2{
    \@tempcnta#1\relax
    \loop
        #2%
        \advance\@tempcnta\m@ne
        \ifnum\@tempcnta>\z@
    \repeat
}

\def\cg@badbar{\errmessage{cgslash commands may only be used inside a combgame command.}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                          %%
%%                      Thermographs                        %%
%%                                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\define@key[cgk]{thermoplot}{left}{\def\cg@plot@left{#1}}
\define@key[cgk]{thermoplot}{right}{\def\cg@plot@right{#1}}
\define@key[cgk]{thermoplot}{top}{\def\cg@plot@top{#1}}
\define@key[cgk]{thermoplot}{bottom}{\def\cg@plot@bottom{#1}}
\define@key[cgk]{thermoplot}{scale}{\def\cg@plot@scale{#1}}
\define@key[cgk]{thermoplot}{axescolor}{\def\cg@plot@axescolor{#1}}
\define@key[cgk]{thermoplot}{clipmargin}{\def\cg@plot@clipmargin{#1}}
\define@key[cgk]{thermoplot}{baseline}{\def\cg@plot@baseline{#1}}
\define@key[cgk]{thermograph}{linecolor}{\def\cg@therm@linecolor{#1}}
\define@key[cgk]{thermograph}{displ}{\def\cg@therm@displ{#1}}

\newlength\cg@xorigin
\newlength\cg@yorigin
\newlength\cg@xsize
\newlength\cg@ysize
\newlength\cg@vcoord
\newlength\cg@tcoord

\newenvironment{thermoplot}[1][]{%
  \setkeys[cgk]{thermoplot}{left=2,right=-2,top=4,bottom=0,scale=1cm,axescolor=gray,clipmargin=6pt,baseline=0.0}%
  \setkeys[cgk]{thermoplot}{#1}%
  \setlength\cg@xorigin{\cg@plot@scale*\cg@plot@left}%
  \setlength\cg@yorigin{-\cg@plot@scale*\cg@plot@bottom}%
  \setlength\cg@xsize{\cg@plot@scale*\cg@plot@left-\cg@plot@scale*\cg@plot@right}%
  \setlength\cg@ysize{\cg@plot@scale*\cg@plot@top-\cg@plot@scale*\cg@plot@bottom}%
  \psset{xunit=-\cg@plot@scale,yunit=\cg@plot@scale}%
  \begin{pspicture}[\cg@plot@baseline](\the\cg@xsize,\the\cg@ysize)%
  {\color{\cg@plot@axescolor}%
   \psaxes[linecolor=\cg@plot@axescolor](\the\cg@xorigin,\the\cg@yorigin)(0,0)(\the\cg@xsize,\the\cg@ysize)}%
  \addtolength{\cg@xsize}{\cg@plot@clipmargin}\addtolength{\cg@ysize}{\cg@plot@clipmargin}%
  \psclip{\psframe[linecolor=white](-\cg@plot@clipmargin,-\cg@plot@clipmargin)(\the\cg@xsize,\the\cg@ysize)}%
}{%
  \endpsclip
  \end{pspicture}%
}%
\newcommand\trajectory[1][]{%
  \setkeys[cgk]{thermograph}{linecolor=black,displ=0pt}%
  \setkeys[cgk]{thermograph}{#1}%
  \def\cg@coords{{<-}}%
  \cg@readcoordsfortrajectory%
}
\newcommand\thermograph[2][]{%
  \setkeys[cgk]{thermograph}{linecolor=black,displ=0pt}%
  \setkeys[cgk]{thermograph}{#1}%
  \def\cg@therm@mast{#2}%
  \cg@starttrajectory%
  }
\def\cg@starttrajectory{%
  \cg@setvcoord{\cg@therm@mast}%
  \cg@settcoord{\cg@plot@top}%
  \addtolength{\cg@vcoord}{\cg@therm@displ}%
  \edef\cg@coords{{<-}(\the\cg@vcoord,\the\cg@tcoord)}%
  \cg@readcoordsfortrajectory%
}
\def\cg@readcoordsfortrajectory{%
  \@ifnextchar(\cg@readcoord%
    {\expandafter\cg@trajectoryline\cg@coords\cg@readnexttrajectory}%
}
\def\cg@trajectoryline{\psline[linecolor=\cg@therm@linecolor]}
\def\cg@readcoord(#1,#2){%
  \cg@setvcoord{#1}%
  \cg@settcoord{#2}%
  \addtolength{\cg@vcoord}{\cg@therm@displ}%
  \edef\cg@coords{\cg@coords(\the\cg@vcoord,\the\cg@tcoord)}%
  \cg@readcoordsfortrajectory%
}
\def\cg@settcoord#1{%
  \setlength\cg@tcoord{\cg@plot@scale*#1-\cg@plot@scale*\cg@plot@bottom}%
}
\def\cg@setvcoord#1{%
  \setlength\cg@vcoord{\cg@plot@scale*\cg@plot@left-\cg@plot@scale*#1}%
}
\def\cg@readnexttrajectory{\@ifnextchar;{\cg@eatsemicolon}{}}
\def\cg@eatsemicolon;{\cg@starttrajectory}



==> cg-board.tex <==
\ProvidesFile{cg-board.tex}
\newif\ifcg@board@trace%\cg@board@tracetrue % for debugging only

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Suggested for loony symbol:
% \usepackage{marvosym}\def\cgloony{\textrm\Moon}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FOR ALL DRAWING COMMANDS, USE pstricks COMMANDS.
%     \psunit IS SET, BUT \unitlength IS NOT SET.
% The general format for defining new board style is:
%   \newboard[options]{boardname}{code}
% There are numerous examples at the end of this file.
% For options, the following are allowed:
%
% code:  A sequence of character, expansion pairs (must have an even number of atoms)
%        default is X,x,L,l all make a black circle
%                   O,o,R,r all make a white circle
%                   .       is an empty square
%        The origin for an expansion is in the center of square; the expandsion is placed in a
%            makebox(0,0) so that any text is centered.
%        When defining a code for characters #, space, $, \, and ~,
%        quote them with a backslash.  (Do not prepend the \ in the
%        board diagram itself, though if you want to use space and \,
%        you'll need spaces=true.)
%
% unit:  Side length of a square (sets pstricks unit, access with \psunit)
% runit, xunit, yunit:  In case you want different x- and y-coordinate scales.
% linewidth:  Sets the pstricks linewidth
%
% text:  Sizing and style commands for text placed on a square.  (Example: StringsAndCoins)

% square:  What do use for a boardsquare.  (Use "square=" for no square.)
%          Default is a 1x1 square.
%          The origin for drawing the board square is in the lower
%          left corner of the square.  You can access counters
%          \cgboardrow and \cgboardcol to, for example, check parities (see Checkers).
% board:  What to draw for the gameboard.  Use counters cgboardrows and cgboardcols.
%         (Rarely needed;  Usually just draw each square individually as above.)
%         (see Hackenbush)
% frame: Put a frame around the board; generally used for debugging so you can see how large the
%         boards box is.
% printname:  (boolean) true means print the gamename under the board.  Default false.
%    (I use this for new games until such time as I've come up with distinctive pieces.)
%
% insert:  Stuff to insert in the diagram in addition to the gameboard.  Used to decorate the board.
% shrink: (boolean) Make the bounding box is .5 units smaller on each side.
% spaces: (boolean) Spaces and newlines are no longer whitespace (see Hex)
% color:  (boolean) Use color (currently implemented in Hackenbush, TopplingDominoes, Push, Shove)
%         Use \ifcgboardcolor to access
% 

% You can set these options in 4 different ways; suppose you are defining a new board named MyBoard.
% (1)  \newboard[...]{MyBoard}   --- When you defined your board
% (2)  \cgboardset{...}          --- This sets keys for all board types
% (3)  \MyBoardset{...}          --- A command is created by \newboard which appends ``set'' to your board name.
% (4)  \MyBoard[...]{xx\\oo\\}   --- When you make your board, you can define options in place.
% Note that the options are set in this order, and that \cgboardset obliterates the previous \cgboardset, and that
% \MyBoardset obliterates the previous \MyBoardset

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newboard
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \cg@board@extendcode\cg@board@basecode
\def\cgnewboard{\newboard}
\define@key[cgk]{board}{unit}{\psset{unit=#1}}
\define@key[cgk]{board}{xunit}{\psset{xunit=#1}}
\define@key[cgk]{board}{yunit}{\psset{yunit=#1}}
\define@key[cgk]{board}{runit}{\psset{runit=#1}}
\define@key[cgk]{board}{linewidth}{\psset{linewidth=#1}}
\define@key[cgk]{board}{text}[]{\def\cg@board@text{#1}}
\define@key[cgk]{board}{square}[\psline(0,0)(1,0)(1,1)(0,1)(0,0)]{\def\cg@board@square{#1}}
\define@key[cgk]{board}{frame}[\fbox]{\def\cg@board@frame{#1}}
\define@key[cgk]{board}{board}[]{\def\cg@board@theboard{#1}}
\define@key[cgk]{board}{printname}{\def\cg@board@printname{#1}}
\define@key[cgk]{board}{code}{\def\cg@board@extendcode{#1}}
\define@key[cgk]{board}{insert}{\def\cg@board@insertion{#1}}
\def\cgboardset#1{\def\cg@board@set{#1}}\def\cg@board@set{}

\define@boolkey[cgk]{board}{shrink}[true]{}
\define@boolkey[cgk]{board}{spaces}[true]{}
\define@boolkey[cgk]{board}{color}[true]{}

\newpsobject{cg@board@dottedline}{psline}{linestyle=dashed,dash=1.5pt 1.5pt}
\def\cg@board@default@keys{
   unit=.3cm,
   linewidth=.5pt,
   text=,
   square={\psline(0,0)(1,0)(1,1)(0,1)(0,0)},
   frame=,
   board=,
   printname=,
   code=,
   insert=,
   shrink=false,
   spaces=false,
   color=false
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Base gameboard code
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\cg@board@basecode{
x {\pscircle*{.45}}
o {\pscircle[fillstyle=solid,fillcolor=white]{.45}}
l {\cgboardalias{x}}
r {\cgboardalias{o}}
0 {0}
1 {1}
2 {2}
3 {3}
4 {4}
5 {5}
6 {6}
7 {7}
8 {8}
9 {9}
. {}
\ {\cgboardalias{.}}
\#{\cgnosquare}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% catcode stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\catcode`\#=11\gdef\cg@sharp{#}}
{\catcode`\$=11\gdef\cg@dollar{$}} % Second copy keeps file
{\catcode`\$=11\gdef\cg@dollar{$}} %  looking pretty in emacs
{\catcode`\~=11\gdef\cg@tilde{~}}
\begingroup
\catcode`|=0\catcode`\\=12|gdef|cg@backslash{\}
|endgroup
\def\cg@board@setcatcodes{%
  \catcode`\#=12%
  \catcode`\^=12%
  \catcode`\|=12%
  \catcode`\[=12%
  \catcode`\]=12%
  \catcode`\~=12\relax%
  \ifcgk@board@spaces
  \catcode`\\=12%
  \catcode`\ =12%
  \catcode`\^^M=12\relax%
  \fi%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Code stuff (i.e., the encoding of characters to board squares)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\cgboardalias#1{%
  \@if@cg@board@code@defined{#1}%
  {\csname cg@board@code@#1\endcsname}%
  {\GenericWarning{}{Warning: Code for ``#1'' (an alias) unknown in game diagram}}}

\def\cg@board@set@code#1#2{
  \ifcg@board@trace\typeout{Setting ``\expandafter\string\csname cg@board@code@#1\endcsname'' to ``(not telling)''}\fi
  \expandafter\def\csname cg@board@code@#1\endcsname{#2}}
\def\cg@board@setstrings#1{\cg@board@buildsetstrings#1\cg@end\cg@end}
\def\cg@board@buildsetstrings#1#2{
  \ifx\cg@end#1
    \ifx\cg@end#2\let\next\relax
    \else\errmessage{combgames error: Mismatched arguments in board codes}
    \fi
  \else
    \ifx\\#1\cg@board@set@code{\cg@backslash}{#2}
    \else\ifx\ #1\cg@board@set@code{\space}{#2}
    \else\ifx#1\#\cg@board@set@code{\cg@sharp}{#2}
    \else\ifx\~#1\cg@board@set@code{\cg@tilde}{#2}
    \else\ifx\$#1\cg@board@set@code{\cg@dollar}{#2}
    \else\cg@board@set@code{#1}{#2}
    \fi\fi\fi\fi\fi
    \let\next\cg@board@buildsetstrings
  \fi
  \next
}

\def\cg@board@set@keys@#1{\expandafter\cg@board@set@keys\expandafter{#1}}
\def\cg@board@set@keys#1{\setkeys[cgk]{board}{#1}}
\newcommand\newboard[3][]{%
  \expandafter\newcommand\csname @cg@board@#2keys\endcsname{}%
  \expandafter\newcommand\csname #2set\endcsname[1]{%
    \expandafter\def\csname @cg@board@#2keys\endcsname{##1}}%
  \expandafter\newcommand\csname#2\endcsname[1][]{%
    %
    \ifmmode\def\cg@board@afterdone{}   % Force math mode if not in math mode
       \else\def\cg@board@afterdone{$}$ % (I forget why, mind you)
    \fi
    \begingroup%
    \expandafter\cg@board@set@keys\expandafter{\cg@board@default@keys}% Keys set in this file
    \setkeys[cgk]{board}{#1}% E.g., \newboard[...]{Domineering}
    \expandafter\cg@board@set@keys\expandafter{\cg@board@set}% \cgboardset{...}
    \expandafter\cg@board@set@keys@\expandafter{\csname @cg@board@#2keys\endcsname}% E.g., Domineeringset{...}
    \setkeys[cgk]{board}{##1}% E.g., \Domineering[...]{xo\\oo}
    \let\ifcgboardcolor=\ifcgk@board@color
    \expandafter\cg@board@buildsetstrings\cg@board@basecode\cg@end\cg@end
    \cg@board@setstrings{#3}%
    \expandafter\cg@board@buildsetstrings\cg@board@extendcode\cg@end\cg@end
    \begingroup%
    \cg@board@setcatcodes%
    \cg@board@read@the@board}}
\def\cg@board@read@the@board#1{\endgroup\cg@board@board{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Scanning and drawing the board
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{cgboardcol}
\newcounter{cgboardrow}
\newcounter{cgboardcols}
\newcounter{cgboardrows}

\def\cg@board@setdims#1{%
  \setcounter{cgboardcols}{0}\setcounter{cgboardcol}{0}\setcounter{cgboardrows}{0}%
                \cg@board@setdims@#1\end}%
\def\cg@board@advancerow{%%
  \ifnum\value{cgboardcols}<\value{cgboardcol} \setcounter{cgboardcols}{\value{cgboardcol}}\fi%
  \ifnum\value{cgboardcol}>0% Ignore leading newline (and the unlikely blank line)%
  \setcounter{cgboardcol}{0}%
  \refstepcounter{cgboardrows}\fi}%

{
\catcode`\^^M=12\relax%
\gdef\cg@board@setdims@#1{%
 \ifx#1\end%%
     \ifnum\value{cgboardcol}>0\cg@board@advancerow\fi% Append missing newline%
     \let\next=\relax%
 \else%
   % The following line must not end in a comment --- testing for newline
    \ifx#1
        \cg@board@advancerow%
    \else\ifx#1\\\cg@board@advancerow%
    \else\refstepcounter{cgboardcol}%
    \fi\fi%
 \let\next=\cg@board@setdims@\fi \next}}%

\def\cg@board@#1{%
  \psset{arrows=-}%
  \ifcgk@board@shrink\cg@board@decrementdims%
  \begin{pspicture}(.5,.5)(\arabic{cgboardcols}.5,\arabic{cgboardrows}.5)%
    \else%
    \begin{pspicture}(\arabic{cgboardcols},\arabic{cgboardrows})%
      \fi%
      \cg@board@theboard%
      \rput(0,-.1){\makebox(0,0)[lt]{\scriptsize\sc \cg@board@printname}}%
      \ifcgk@board@shrink\cg@board@incrementdims\fi%
      \cg@board@process{#1}%
      \cg@board@insertion%
    \end{pspicture}}%

\def\cg@board@incrementdims{%
  \addtocounter{cgboardrows}{1}%
  \addtocounter{cgboardcols}{1}}

\def\cg@board@decrementdims{%
  \addtocounter{cgboardrows}{-1}%
  \addtocounter{cgboardcols}{-1}}

\def\cg@board@process#1{%
  \setcounter{cgboardrow}{\value{cgboardrows}} \setcounter{cgboardcol}{0}  %
  \cg@board@process@#1\end%%
}
{
\catcode`\^^M=12\relax%
  \gdef\cg@board@process@#1{%
    \ifx#1\end%
  \let\next=\relax%
  \else%
   % first adjust row, col%
   % The following line must not end in a comment --- testing for newline
   \ifx#1
   \ifnum\value{cgboardcol}>0% Ignore leading newline (and the unlikely blank line)%
   \addtocounter{cgboardrow}{-1}\fi%
     \setcounter{cgboardcol}{0}%
   \else%
   \ifx#1\\%
   \ifnum\value{cgboardcol}>0% Ignore leading newline (and the unlikely blank line)%
   \addtocounter{cgboardrow}{-1}\fi%
     \setcounter{cgboardcol}{0}%
   \else%
     \addtocounter{cgboardcol}{1}%
   % what gets drawn is game specific
   \cg@board@displaychar{#1}%
   \fi\fi%
   % continue looping%
 \let\next=\cg@board@process@\fi \next}}%

\newlength{\cg@board@halfunit}

\def\cg@board@board#1{%
  \cg@board@setdims{#1}%
  \ifcgk@board@shrink\cg@board@decrementdims\fi%
  \setlength{\cg@board@halfunit}{.5\psyunit}%
  \setlength{\cg@board@halfunit}{\value{cgboardrows}\cg@board@halfunit}%
  \ifcgk@board@shrink\cg@board@incrementdims\fi%
  \raisebox{.5ex}{\raisebox{-1\cg@board@halfunit}%%
    {\expandafter\cg@board@frame%
      {\cg@board@%
        {#1}}}}\endgroup\cg@board@afterdone}%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Processing characters of a cgboard
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@if@cg@board@code@defined#1#2#3{{\@ifundefined{cg@board@code@#1}{#3}{#2}}}

\def\cg@board@displaychar#1{%
  \@if@cg@board@code@defined{#1}%
  {\cg@board@display@char@#1}%
  {\lowercase{\@if@cg@board@code@defined{#1}}%
    {\lowercase{\cg@board@display@char@#1}}%
    {\GenericWarning{}{Warning: Code for ``#1'' unknown in game diagram}}}}

\newif\ifcg@board@drawsquare
\def\cgnosquare{\global\cg@board@drawsquarefalse}

\def\cg@board@display@char@#1{%
  \rput(\value{cgboardcol},\value{cgboardrow}){%
    \cg@board@drawsquaretrue%
    \rput(-.5,-.5){\makebox(0,0){\cg@board@text%
        {\ifcg@board@trace\typeout{Expanding ``\expandafter\string\csname cg@board@code@#1\endcsname''}\fi%
          \csname cg@board@code@#1\endcsname}}}%
    \rput(-1,-1){\ifcg@board@drawsquare\cg@board@square\fi}}}

\def\cg@board@drawsquare{{\rput(-.5,-.5){\cg@board@square}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THE GAMES DEFINED
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DOMINEERING%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newboard[unit=.3cm,square=]{Domineering}{%%
  o {{\psline(-.5,-.5)(.5,-.5)(.5,.5)(-.5,.5)(-.5,-.5)}}%
  x {{\rput(0,0){{\pspolygon*[linewidth=0pt,linecolor=lightgray](-.5,-.5)(-.5,.5)(.5,.5)(.5,-.5)}}%
      \psline(-.5,-.5)(.5,-.5)(.5,.5)(-.5,.5)(-.5,-.5)}}%
  ^ {}%
  > {}%
  v {\psline(-.5,-.5)(.5,-.5)(.5,1.5)(-.5,1.5)(-.5,-.5)%%
      \rput(-.5,-.5){\pspolygon*[linewidth=0pt]%%
      (.4,.4)(.2,.2)(.8,.2)(.6,.4)(.6,1.6)(.8,1.8)(.2,1.8)(.4,1.6)}}%
  < {{\psline(-.5,-.5)(1.5,-.5)(1.5,.5)(-.5,.5)(-.5,-.5)}%
      \rput(-.5,-.5){\pspolygon*[linewidth=0pt]%
       (.4,.4)(.2,.2)(.2,.8)(.4,.6)(1.6,.6)(1.8,.8)(1.8,.2)(1.6,.4)}}%%
 }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CLOBBER
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Clobber@Base#1#2{
  \SpecialCoor
  \rput(-.5,-.5){
    \psset{offset=0,nodesep=.1}
    \ifx#2a
    \pnode(.13333,.75){a}
    \pnode(.86666,-1|a){b}
    \pnode(.73333,.25){c}
    \pnode(.26666,-1|c){d}
    \pnode([angle=0]a){at}
    \pnode([angle=0]d){dt}
    \pnode([angle=-71.565,nodesep=.1]a){a1}
    \pnode([angle=180,nodesep=.05]c){c1}
    \pnode([angle=71.565]c){c2}
    \pnode([angle=108.435,nodesep=.1]dt){d2}
    \pnode([angle=-71.565,nodesep=.00]at){a2}
    \psarc(.5,.22){.08}{-240}{60}
    \else
    \pnode(.13333,.25){a}
    \pnode(.86666,-1|a){b}
    \pnode(.73333,.75){c}
    \pnode(.26666,-1|c){d}
    \pnode([angle=0]a){at}
    \pnode([angle=0]d){dt}
    \pnode([angle=71.565,nodesep=.1]a){a1}
    \pnode([angle=180,nodesep=.05]c){c1}
    \pnode([angle=-71.565]c){c2}
    \pnode([angle=-108.435,nodesep=.1]dt){d2}
    \pnode([angle=71.565,nodesep=.00]at){a2}
    \psarc(.5,.78){.08}{-60}{240}
    \fi
    \ifx#1O
    \pspolygon[linearc=.00](a1)(a2)(b)(c2)(c1)(d)
    \psset{linewidth=.015\psunit}
    \else
    \pspolygon[linearc=.00](a1)(a2)(b)(c2)(c1)(d)
    \pspolygon*[linearc=.00](a1)(a2)(b)(c2)(c1)(d)
    \psset{linecolor=white,linewidth=.5\pslinewidth}
    \fi
    \psline(d)(d2)(c2)(d2)(a2)
  }
}
\def\ClobberO{\Clobber@Base{O}{c}}
\def\ClobberX{\Clobber@Base{X}{c}}
\newboard[unit=.5cm]{Clobber}{
  x {\ClobberX}
  o {\ClobberO}
}
\newboard[unit=.3cm]{AntiClobber}{
  x {\Clobber@Base{X}{a}}
  o {\Clobber@Base{O}{a}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% DOTS AND BOXES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newboard[square=,unit=.35cm,shrink=true,text=\bf]{DotsAndBoxes}{
  o {\pscircle*{.3}}
  - {\psline(-1,0)(1,0)\rput(-1,0){\cgboardalias{o}}}
  | {\psline(0,-1)(0,1)\rput(0,-1){\cgboardalias{o}}}
  : {\cg@board@dottedline(0,-1)(0,1)\rput(0,-1){\cgboardalias{o}}}
  + {\cg@board@dottedline(-1,0)(1,0)\rput(-1,0){\cgboardalias{o}}}
  * {\rput(-.05,0){\makebox(0,0){{$\cgloony$}}}}
  A {A}
  B {B}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% STRINGS AND COINS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\StringsAndCoinsCoin#1{\rput(0,0){#1}\rput(0,0){\pscircle{.5}}}
\newboard[square=,unit=.35cm,text=\bf\footnotesize]{StringsAndCoins}{
 o {\StringsAndCoinsCoin{\rm\$}}
 + {\cg@board@dottedline(-.45,0)(.45,0)}
 : {\cg@board@dottedline(0,-.45)(0,.45)}
 | {\psline(0,-.45)(0,.45)}
 * {\psline(-.45,0)(.45,0)\rput(-.05,.075){\makebox(0,0)[b]{$\cgloony$}}}
 - {\psline(-.45,0)(.45,0)}
 ! {\psline(0,-.45)(0,.45)\rput(-.05,0){\makebox(0,0)[l]{$\cgloony$}}}
 A {\StringsAndCoinsCoin{A}}
 B {\StringsAndCoinsCoin{B}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CHOMP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ChompPoison{\pscircle{.3}\psline(-.3,-.3)(.3,.3)\psline(-.3,.3)(.3,-.3)}
\newboard{Chomp}{
  o {}
  x {\cgboardalias{p}}
  p {\ChompPoison}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BRIDGIT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newboard[shrink=true,square=]{Bridgit}{
  o {\rput(0,0){\pscircle{.2}}}
  x {\rput(0,0){\pscircle*{.2}}}
  - {\psline(-.8,0)(.8,0)}
  | {\psline(0,-.8)(0,.8)}
  + {\cg@board@dottedline(-.8,0)(.8,0)}
  : {\cg@board@dottedline(0,-.8)(0,.8)}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AMAZONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\AmazonsArcher{%
  \psline[arrowsize=1\pslinewidth]{->}(.25,.25)(.8,.8)%
  \psline(.25,.8)(.3,.3)(.8,.25)%
  \psline[linewidth=1.5\pslinewidth](.2,.23)(.25,.25)(.23,.2)%
  \pscurve[linewidth=2\pslinewidth](.2,.8)(.675,.675)(.8,.2)}%
\def\AmazonsR{{\pscircle{.45}}\rput(-.5,-.5){\AmazonsArcher}}
\def\AmazonsL{{\pscircle*{.45}}{\psset{linecolor=white}\rput(-.5,-.5){\AmazonsArcher}}}
\newboard{Amazons}{
  o {}
  x {{\rput(0,0){{\pspolygon*[linewidth=0pt,linecolor=lightgray](-.5,-.5)(-.5,.5)(.5,.5)(.5,-.5)}}%
      \psline(-.5,-.5)(.5,-.5)(.5,.5)(-.5,.5)(-.5,-.5)}}%
  l {\AmazonsL}
  r {\AmazonsR}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SHOVE and PUSH
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\PushBase#1#2#3{
  \def\doit##1{%
    \ifcgboardcolor%
    \ifx#2O\pscurve*[linecolor=red]##1\pscurve##1%
    \else\ifx#2X\pscurve*[linecolor=blue]##1\pscurve##1%
    \else\pscurve*[linecolor=green]##1\pscurve##1%
    \fi\fi\else%
    \ifx#2O\pscurve##1%
    \else\ifx#2X\pscurve*##1%
    \else\pscurve*[linecolor=lightgray]##1\pscurve##1%
    \fi\fi\fi
  }
  \def\thepiece{
    \doit{(.55,.1)(.42,.2)(.33,.27)(.32,.3)(.33,.4)(.33,.5)(.33,.56)(.34,.6)(.355,.625)(.39,.625)
    (.39,.625)(.39,.625)(.39,.625)(.41,.8)(.425,.83)(.45,.83)(.465,.8)(.5,.4)(.525,.3)(.625,.22)}
    \ifx#2X
    \psecurve[linecolor=white,linewidth=.5\pslinewidth](.355,.625)(.39,.625)(.4,.6)(.4,.415)(.4,.425)
    \else
    \psecurve(.355,.625)(.39,.625)(.4,.6)(.4,.415)(.4,.425)
    \fi
    \psset{linewidth=.5\pslinewidth}
    \ifx#1P
    \psline(.6,.4)(.7,.4)
    \psline(.6,.7)(.7,.7)
    \else
    \psline(.7,.3)(.85,.3)
    \psline(.65,.45)(.9,.45)
    \psline(.65,.6)(.8,.6)
    \psline(.65,.75)(.9,.75)
    \fi}
  {
  \ifx#3a\psset{unit=.6\psunit}\fi
  \ifx#1P\rput(-.5,-.5){\thepiece}\else\rput(-.6,-.5){\thepiece}\fi
  }
}
\def\PushO{\PushBase{P}{O}{.}}
\def\PushX{\PushBase{P}{X}{.}}
\def\PushG{\PushBase{P}{G}{.}}
\def\ShoveO{\PushBase{S}{O}{.}}
\def\ShoveX{\PushBase{S}{X}{.}}
\def\ShoveG{\PushBase{S}{G}{.}}
\def\AllSmallPushO{\PushBase{P}{O}{a}}
\def\AllSmallPushX{\PushBase{P}{X}{a}}
\def\AllSmallPushG{\PushBase{P}{G}{a}}
\def\AllSmallShoveO{\PushBase{S}{O}{a}}
\def\AllSmallShoveX{\PushBase{S}{X}{a}}
\def\AllSmallShoveG{\PushBase{S}{G}{a}}
\newboard[unit=.5cm,square={\psline(0,0)(1,0)(1,1)(0,1)}]{Push}{
  . {}
  o {\PushO}
  O {\PushO}
  x {\PushX}
  X {\PushX}
  L {\PushX}
  R {\PushO}
  G {\PushG}
}
\newboard[unit=.5cm,square={\psline(0,0)(1,0)(1,1)(0,1)}]{Shove}{
  . {}
  o {\ShoveO}
  x {\ShoveX}
  g {\ShoveG}
}
\newboard[unit=.5cm,square={\psline(0,0)(1,0)(1,1)(0,1)}]{AllSmallShove}{
  . {}
  o {\AllSmallShoveO}
  x {\AllSmallShoveX}
  g {\AllSmallShoveG}
}
\newboard[unit=.5cm,square={\psline(0,0)(1,0)(1,1)(0,1)}]{AllSmallPush}{
  . {}
  o {\AllSmallPushO}
  x {\AllSmallPushX}
  g {\AllSmallPushG}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% HACKENBUSH STRINGS%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\hackred#1{%
  \ifcgboardcolor{\psset{linecolor=red,linewidth=4\pslinewidth}#1}%
  \else{\psset{doubleline=true,doublesep=1pt,linewidth=.5pt}#1}\fi}%
\def\hackblue#1{%
  \ifcgboardcolor{\psset{linecolor=blue,linewidth=4\pslinewidth}#1}%
  \else{\psset{linewidth=4\pslinewidth}#1}\fi}%
\def\hackgreen#1{%
  \ifcgboardcolor{\psset{linecolor=green,linewidth=4\pslinewidth}#1}%
  \else{\psset{linewidth=4\pslinewidth,linecolor=lightgray}#1}\fi}%

\def\hackedge{\psline(-.5,0)(.5,0)}
\def\Hackenbushstring@frame#1{\hspace{.15\psunit}#1\hspace{.15\psunit}}
\newboard[frame=\Hackenbushstring@frame,square={\rput(0,.5){\pscircle*{.15}}},unit=.5cm,xunit=.8cm,yunit=.3cm,%
         board={\psline[linewidth=8\pslinewidth,linecolor=lightgray](0,-.25)(0,\arabic{cgboardrows}.25)}]%
    {Hackenbushstring}{
  o {\hackred{\hackedge}\rput(.5,0){\pscircle*{.15}}\rput(-.5,0){\pscircle*{.15}}}
  x {\hackblue{\hackedge}\rput(.5,0){\pscircle*{.15}}\rput(-.5,0){\pscircle*{.15}}}
  b {\cgboardalias{x}}
  g {\hackgreen{\hackedge}\rput(.5,0){\pscircle*{.15}}\rput(-.5,0){\pscircle*{.15}}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TOPPLING DOMINOES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\DOMINO#1#2#3{\pspolygon#1[#3](-.2,-.5)(-.2,.3)(0,.5)(0,-.5)%
              \pspolygon#1[#3](0,-.5)(0,.5)(.2,.5)(.2,-.5)%
              \psline[#2](0,0)(-.2,-.1)}
\newboard[xunit=.3cm,yunit=.6cm,square=,%
         board={\psline[linewidth=6\pslinewidth,linecolor=lightgray](0,0)(\arabic{cgboardcols},0)}]
        {TopplingDominoes}{
          x {\ifcgboardcolor\DOMINO{}{}{fillcolor=blue,fillstyle=solid}\else\DOMINO{*}{linecolor=white}{}\fi}
          o {\ifcgboardcolor\DOMINO{}{}{fillcolor=red,fillstyle=solid}\else\DOMINO{}{}{}\fi}
          g {\ifcgboardcolor\DOMINO{}{}{fillcolor=green,fillstyle=solid}\else\DOMINO{}{}{fillcolor=lightgray,fillstyle=solid}\fi}
        }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% HEX
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\HexHexagon{\rput(0,0){\psline(-.666666,0)(-.333333,1)(.333333,1)(.666666,0)(.3333333,-1)(-.3333333,-1)(-.666666,0)}}
\def\HexBlack{\rput(0,0){\pscircle*{.5}}}
\def\HexWhite{\rput(0,0){\pscircle{.5}}\rput(0,0){\pscircle{.2}}}
\newlength{\Hexunit}
\setlength{\Hexunit}{.125cm}
\newboard[square=,runit=1.3\Hexunit,xunit=1.73206\Hexunit,yunit=1\Hexunit,spaces]{Hex}{
  o {\HexHexagon}
  * {\HexHexagon}
  l {\HexBlack}
  r {\HexWhite}
  x {\HexHexagon\HexBlack}
  o {\HexHexagon\HexWhite}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MAZE and MAIZE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newboard[square=,unit=.2cm,shrink,spaces]{Maze}{
  L {$\L$} R {$\R$} N {$\N$} P {$\P$}
  o {}
  * {\psline(-.05,-.05)(.05,.05)\psline(-.05,.05)(.05,-.05)}
  x {\pscircle{.8}\rput(0,0){\rput(0,0){$\star$}}}
  / {\psline(-1,-1)(1,1)}
 \\ {\psline(-1,1)(1,-1)}
}
\newboard[square=,unit=.2cm,shrink,spaces]{Maize}{
  L {$\L$} R {$\R$} N {$\N$} P {$\P$}
  o {}
  * {\psline(-.05,-.05)(.05,.05)\psline(-.05,.05)(.05,-.05)}
  x {\pscircle{.8}\pscircle*{.1}}
  / {\psline(-1,-1)(1,1)}
 \\ {\psline(-1,1)(1,-1)}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CHECKERS
% Checkers is not yet complete --- needs a King --- provided here only
%  to provide an example of using counters cgboardrow and cgboardcol
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\CheckersSquare{ 
  \@tempcnta=\value{cgboardrow}
  \advance\@tempcnta\value{cgboardcol}
  \ifodd\@tempcnta
  {\pspolygon(0,0)(1,0)(1,1)(0,1)}\else
  {\pspolygon[fillcolor=lightgray,fillstyle=solid](0,0)(1,0)(1,1)(0,1)}\fi
}

\newboard[square=.]{Checkers}{ % Since a square is drawn after the
  % piece, Checkers requires us to draw the square explicitly.
  . {\rput(-.5,-.5){\CheckersSquare}}
  x {\cgboardalias{.}\pscircle*{.4}}
  o {\cgboardalias{.}\pscircle[fillstyle=solid,fillcolor=white]{.4}}
}


==> cg-sym.tex <==
\ProvidesFile{cg-sym.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                          %%
%%                    Font Declarations                     %%
%%                                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareFontFamily{OT1}{cgames}{}
\DeclareFontShape {OT1}{cgames}{m}{n}{<-6> game5 <6-7> game6 <7-8> game7 <8-9> game8 <9-10> game9 <10-> game10}{}
\DeclareSymbolFont{cgsymb}{OT1}{cgames}{m}{n}

\DeclareMathSymbol{\cgup}        {\mathord}  {symbols}{"22}
\DeclareMathSymbol{\cgdown}      {\mathord}  {symbols}{"23}
\DeclareMathSymbol{\cgdoubleup}  {\mathord}  {symbols}{"2A}
\DeclareMathSymbol{\cgdoubledown}{\mathord}  {symbols}{"2B}
\DeclareMathSymbol{\cgneg}       {\mathord}  {symbols}{"00}
\DeclareMathSymbol{\cgstar}      {\mathord}  {symbols}{"03}
\DeclareMathSymbol{\cgtripleup}  {\mathord}  {cgsymb} {"00}
\DeclareMathSymbol{\cgtripledown}{\mathord}  {cgsymb} {"01}
\DeclareMathSymbol{\cgquadup}    {\mathord}  {cgsymb} {"02}
\DeclareMathSymbol{\cgquaddown}  {\mathord}  {cgsymb} {"03}
\DeclareMathSymbol{\cgtiny}      {\mathord}  {cgsymb} {"08}
\DeclareMathSymbol{\cgminy}      {\mathord}  {cgsymb} {"09}
\DeclareMathSymbol{\cgnmultiply} {\mathrel}  {cgsymb} {"0A}
\DeclareMathSymbol{\cgfuzzy}     {\mathrel}  {cgsymb} {"0B}
\DeclareMathSymbol{\cglfuz}      {\mathrel}  {cgsymb} {"0C}
\DeclareMathSymbol{\cggfuz}      {\mathrel}  {cgsymb} {"0D}
\DeclareMathSymbol{\cgupsum}     {\mathrel}  {cgsymb} {"0E}
\DeclareMathSymbol{\cgdownsum}   {\mathrel}  {cgsymb} {"0F}
\DeclareMathSymbol{\cgko}        {\mathord}  {cgsymb} {"10}
\DeclareMathSymbol{\cgKo}        {\mathord}  {cgsymb} {"11}
\DeclareMathSymbol{\cgbarforko}  {\mathord}  {cgsymb} {"12}
\DeclareMathSymbol{\cgfarstar}   {\mathord}  {cgsymb} {"13}
\DeclareMathSymbol{\cgloony}     {\mathord}  {cgsymb} {"14}
\DeclareMathSymbol{\cgsunny}     {\mathord}  {cgsymb} {"15}

\newcommand{\cgkobar}{\cgbarforko\cgko}
\newcommand{\cgKobar}{\cgbarforko\cgKo}

\newcommand\cgups[1]{%
  \ifcase#1\relax%
    0\or\cgup\or\cgdoubleup\or\cgtripleup\or\cgquadup%
  \else%
    \ifnum#1<\z@\cg@updownerror\else{#1}\cdot\cgup\fi%
  \fi%
}
\newcommand\cgdowns[1]{%
  \ifcase#1\relax%
    0\or\cgdown\or\cgdoubledown\or\cgtripledown\or\cgquaddown%
  \else%
    \ifnum#1<\z@\cg@updownerror\else{#1}\cdot\cgup\fi%
  \fi%
}
\newcommand\cg@updownerror{\errmessage{Argument to cgups and cgdowns must be positive.}}



==> cg-tree.tex <==
\ProvidesFile{cg-tree.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                          %%
%%                      Game Trees                          %%
%%                                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Some rather complicated logic for an analogue of \futurelet that skips over spaces:

\def\cg@fletnosp#1#2{\def\@tempa{#1}\def\@tempb{#2}\futurelet\@tempc\cg@fletnosp@}
\def\cg@fletnosp@{\ifx\@tempc\@sptoken\let\@tempd\cg@fletnosp@@\else\expandafter\let\@tempa\@tempc\let\@tempd\@tempb\fi\@tempd}
{\def\:{\cg@fletnosp@@} \expandafter\gdef\: {\futurelet\@tempc\cg@fletnosp@}}

\define@key[cgk]{cgtree}{arrows}{\def\cg@tree@arrows{#1}}
\define@key[cgk]{cgtree}{unit}{\def\cg@tree@unit{#1}}
\define@key[cgk]{cgtree}{nodesep}{\def\cg@tree@nodesep{#1}}
\define@key[cgk]{cgnode}{arrow}{\def\cg@node@arrow{#1}}
\define@key[cgk]{cgnode}{sep}{\def\cg@node@sep{#1}}
\define@key[cgk]{cgnode}{name}{\def\cg@node@name{#1}}
\define@boolkey[cgk]{cgnode}{ko}[true]{}

\newcounter{cg@nextnodeord}  % Global node ordinal counter for default names

\newcommand\cgtree[2][]{{
  \setkeys[cgk]{cgtree}{arrows=-,nodesep=.75ex,unit=1cm}
  \setkeys[cgk]{cgtree}{#1}
  \cg@gtinit%
  \cg@gtprocessnode#2\cg@gtend%
}}

\def\cg@gtinit{
  \newcount\cg@gtx
  \newcount\cg@gty
  \newcount\cg@gtnextx
  \newcount\cg@gtnexty
  \newcount\cg@gtparentx
  \newcount\cg@gtparenty
  \newcount\cg@gtxadjustment
  \newif\ifcg@gtleft
  \def\cg@node@psep{0pt}
  \def\cg@node@pname{none}
  \psset{unit=\cg@tree@unit}
}

\def\cg@gtend{@@@ENDCGTREE@@@}

\def\cg@gtprocessnode#1{\@ifnextchar[{\cg@gtprocessnode@{#1}}{\cg@gtprocessnode@{#1}[]}}
\def\cg@gtprocessnode@#1[#2]{
  \stepcounter{cg@nextnodeord}
  \setkeys[cgk]{cgnode}{arrow=\cg@tree@arrows,sep=\cg@tree@nodesep,ko=false,name=cggt\arabic{cg@nextnodeord}}
  \ifx.\cg@gtnextchar\def\cg@node@sep{0pt}\fi   % Override default for empty entry
  \setkeys[cgk]{cgnode}{#2}
  \ifx:\cg@gtnextchar
    % Symbolic link: don't change nextx/nexty OR render the node OR try a subtree.
    \let\next=\cg@gtprocesschar
  \else
    \ifcgk@cgnode@ko
      \cg@gtx=\the\cg@gtparentx
      \cg@gty=\the\cg@gtparenty
      \advance\cg@gtx by \ifcg@gtleft-\fi \the\cg@gtxadjustment
      \advance\cg@gtx by\ifcg@gtleft -3\else 3\fi
    \else
      \cg@gtx=\the\cg@gtnextx
      \cg@gty=\the\cg@gtnexty
      \advance\cg@gtx by \ifcg@gtleft-\fi \the\cg@gtxadjustment
      \cg@gtnextx=\the\cg@gtx
      \advance\cg@gtnextx by \ifcg@gtleft -2\else 2\fi
    \fi
    \cg@gtshow{\ifx.\cg@gtnextchar\else#1\fi}
    \let\next=\cg@gttrysubtree
    \cg@gtxadjustment=0
  \fi
  \cg@gtdrawline
  \next
}

\def\cg@gttrysubtree{
  \@ifnextchar({\cg@gtstartsubtree}{\cg@gtprocesschar}
}

\def\cg@gtstartsubtree({
  \begingroup
  \cg@gtparentx=\the\cg@gtx
  \cg@gtparenty=\the\cg@gty
  \cg@gtnextx=\the\cg@gtparentx
  \cg@gtnexty=\the\cg@gtparenty
  \advance\cg@gtnextx by -1
  \advance\cg@gtnexty by -2
  \cg@gtlefttrue
  \edef\cg@node@psep{\cg@node@sep}
  \edef\cg@node@pname{\cg@node@name}
  \cg@gtprocesschar
}

\def\cg@gtprocesschar{\cg@fletnosp\cg@gtnextchar\cg@gtprocesschar@}
\def\cg@gtprocesschar@#1{
  \ifx\cg@gtend\cg@gtnextchar
    \let\next=\relax
  \else\ifx(\cg@gtnextchar
    \errmessage{Unexpected (}
  \else\ifx|\cg@gtnextchar
    \ifcg@gtleft
      \cg@gtleftfalse
      \cg@gtnextx=\the\cg@gtparentx
      \cg@gtnexty=\the\cg@gtparenty
      \advance\cg@gtnextx by 1
      \advance\cg@gtnexty by -2
      \let\next=\cg@gtprocesschar
    \else\errmessage{Extra | in gametree description.}
    \fi
  \else\ifx+\cg@gtnextchar
    \advance\cg@gtxadjustment by 1
    \let\next=\cg@gtprocesschar
  \else\ifx-\cg@gtnextchar
    \advance\cg@gtxadjustment by -1
    \let\next=\cg@gtprocesschar
  \else\ifx)\cg@gtnextchar
    \ifcg@gtleft\errmessage{Missing | in gametree description.}
    \else
      \let\next=\cg@gtendsubtree
    \fi
  \else
    \def\next{\cg@gtprocessnode{#1}}
  \fi\fi\fi\fi\fi\fi
  \next
}

\def\cg@gtendsubtree{
  \endgroup\cg@gtprocesschar
}

\def\cg@gtshow#1{
  \rput(\the\cg@gtx,\the\cg@gty)
    {\expandafter\rnode{\cg@node@name}{$#1$}}
}

\def\cg@gtdrawline{{
  \psset{arrows=\cg@node@arrow,nodesepA=\cg@node@psep,nodesepB=\cg@node@sep}
  \ifcgk@cgnode@ko
    \ifcg@gtleft\def\cg@gtangle{20}\else\def\cg@gtangle{-20}\fi
    \ncarc[arcangleA=\cg@gtangle,arcangleB=\cg@gtangle]{\cg@node@pname}{\cg@node@name}
  \else
    \ncline{\cg@node@pname}{\cg@node@name}
  \fi
}}




==> graphs_config.tex <==
% Local configuration for version 1.53 of graphs.sty. Frank Drewes, 16.11 2003

% The \special macro below must contain the path under which the file
% graphs.header can be found in you local installation. Please modify it
% accordingly.

\special{header=graphs.header}


==> graphs_ps.tex <==
% `special' commands for version 1.53 of graphs.sty. Frank Drewes, 16/11 2003

\def\ps@s{ }
\def\ps@convertnum#1{
	#1 \number\unitlength\ps@s mul 65536 div 72.27 div 72 mul
}

%-----------------------------------------------------------------------------%


\def\ps@rectangle[#1,#2]{% width, height
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		[ \g@ncolour\ps@s\g@ncolourmod ]\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\iffillednodes true \else false\fi\ps@s
		psrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@circle[#1]{% diameter
\special{"	\ps@convertnum{#1}
		[ \g@ncolour\ps@s\g@ncolourmod ]\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\iffillednodes true \else false\fi\ps@s
		pscircle}}

%-----------------------------------------------------------------------------%

\def\ps@line(#1,#2){% end x, end y
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\g@ldash\ps@s
		psline}}

%-----------------------------------------------------------------------------%

\def\ps@loopA(#1,#2)(#3,#4){% from (#1,#2) to (#3,#4)
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psloop}}

%-----------------------------------------------------------------------------%

\def\ps@loopB#1(#2,#3){% angle #1, axis (#2,#3)
\special{"	#1
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		psloopbyangle
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psloop}}
		
%-----------------------------------------------------------------------------%

\def\ps@looparrowonrectangleA(#1,#2)(#3,#4)[#5,#6]{% 
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		\ps@convertnum{#5}
		\ps@convertnum{#6}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowonrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@looparrowoncircleA(#1,#2)(#3,#4)[#5]{% 
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		\ps@convertnum{#5}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@looparrowonrectangleB#1(#2,#3)[#4,#5]{% 
\special{"	#1
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		psloopbyangle
		\ps@convertnum{#4}
		\ps@convertnum{#5}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowonrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@looparrowoncircleB#1(#2,#3)[#4]{% 
\special{"	#1
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		psloopbyangle
		\ps@convertnum{#4}
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		pslooparrowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@deletebox(#1,#2){% width, height in scaled points
\special{"	#1 65536 div
		#2 65536 div
		psdeletebox}}

%-----------------------------------------------------------------------------%

\def\ps@arrowonrectangle(#1,#2) [#3,#4]{% x, y, width, height
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psarrowonrectangle}}

%-----------------------------------------------------------------------------%

\def\ps@arrowoncircle(#1,#2) [#3]{% x, y, diameter of circle
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		\g@ldash\ps@s
		psarrowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@path(#1,#2)#3{% start coordinates, (xi,yi[,di]) ...
	\def\extractvalues(##1)##2;{%
	  \ifx\endmarker##1\else%
	    \extractvalues##2;\extractvals(##1,0,)%
	  \fi}%
	\def\extractvals(##1,##2,##3,##4){%
	  \ps@convertnum{##1}%
	  \ps@convertnum{##2}%
	  ##3%
	}%
	\special{" mark \extractvalues#3(\endmarker);
			\ps@convertnum{#1}
			\ps@convertnum{#2}
			\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
			[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
			\g@ldash\ps@s
			[ \g@fcolour\ps@s\g@fcolourmod ]\ps@s
			\iffilledareas true \else false\fi\ps@s pspath}}

%-----------------------------------------------------------------------------%

\def\ps@curve#1#2{% base length, (x1,y1,ang1[factor1]) ...
	\def\extractvalues(##1(##2;##3{%
	  \ifx\endmarker##1\else%
	    \extractvalues(##2;{##3}\extractvals(##1[##3,##3];%
	  \fi}%
	\def\extractvals(##1,##2,##3)[##4,##5]##6;{%
	  ##5\ps@s
	  ##4\ps@s
	  ##3\ps@s
	  \ps@convertnum{##2}%
	  \ps@convertnum{##1}%
	}%
	\special{" mark \extractvalues#2(\endmarker(;{#1}
			\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
			[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
			\g@ldash\ps@s
			[ \g@fcolour\ps@s\g@fcolourmod ]\ps@s
			\iffilledareas true \else false\fi\ps@s pscurve}}

%-----------------------------------------------------------------------------%

\def\ps@bubble#1#2{% length factor, (x1,y1) ...
	\def\extractvalues(##1)##2;{%
	  \ifx\endmarker##1\else%
	    \extractvalues##2;\extractvals(##1)%
	  \fi}%
	\def\extractvals(##1,##2){%
	  \ps@convertnum{##2}%
	  \ps@convertnum{##1}%
	}%
	\special{" mark \extractvalues#2(\endmarker);
			#1\ps@s
			\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
			[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
			\g@ldash\ps@s
			[ \g@fcolour\ps@s\g@fcolourmod ]\ps@s
			\iffilledareas true \else false\fi\ps@s psbubble}}

%-----------------------------------------------------------------------------%

\def\ps@dirbowoncircle(#1,#2)(#3,#4,#5)[#6]{% (x1,x2) (y1,y2,d), radius
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		#5\ps@s
		\ps@convertnum{#6}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\g@ldash\ps@s
		psdirbowoncircle}}

%-----------------------------------------------------------------------------%

\def\ps@dirbowonrectangle(#1,#2)(#3,#4,#5)[#6,#7]{% (x1,x2) (y1,y2,d),
                                                  % xsize, ysize
\special{"	\ps@convertnum{#1}
		\ps@convertnum{#2}
		\ps@convertnum{#3}
		\ps@convertnum{#4}
		#5\ps@s
		\ps@convertnum{#6}
		\ps@convertnum{#7}
		\ps@convertnum{\g@alength}\g@alengthmod\ps@s
		\g@awidth\ps@s\g@awidthmod\ps@s
		\g@atype\ps@s
		\ps@convertnum{\g@lwidth}\g@lwidthmod\ps@s
		[ \g@lcolour\ps@s\g@lcolourmod ]\ps@s
		\g@ldash\ps@s
		psdirbowonrectangle}}

%-----------------------------------------------------------------------------%


